Learning Global Motion with Compact Gaussians for Feed-Forward 4D Reconstruction

Dynamic scene reconstruction from monocular video remains a fundamental challenge in computer vision. Existing feed-forward methods predict 3D Gaussians pixel-wise for each frame, suffering from duplicated Gaussians and view-dependent biases that hinder effective learning of scene motion. We present C4G, a feed-forward 4D reconstruction framework built upon a compact set of timestamp-conditioned learnable Gaussian query tokens. Each token aggregates corresponding features across the full temporal context and decodes a 3D Gaussian whose position is modulated by the target timestamp, enabling globally coherent motion modeling without per-scene optimization. To capture fine-grained details, we further introduce a video diffusion model-based rendering enhancement module. Since our framework effectively aggregates features into Gaussians, we extend this capability to feature lifting, producing a 4D feature field that supports point tracking and dynamic scene understanding. C4G achieves strong novel-view synthesis performance using significantly fewer Gaussians and without requiring camera poses, while exhibiting stronger motion modeling and robustness to large temporal gaps.

==> table/ablation_studies_loss.tex <==

\begin{table}[t]
    \centering
    \caption{\textbf{Ablation studies on loss function.}}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc}
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{DyCheck~\cite{gao2022monocular}} & \multicolumn{3}{c}{TUM-Dynamics~\cite{sturm2012benchmark}} \\
         & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
        \midrule \midrule
        Ours & \textbf{15.54} & \textbf{0.383} & \textbf{0.385} & 18.94 & \textbf{0.575} & \textbf{0.341}\\
        w/o $\mathcal{L}_{\text{track}}$ & 15.46& 0.381& 0.390& \textbf{18.97}& 0.574& 0.342\\
        w/o $\mathcal{L}_\text{depth}$ & 15.50& 0.381& \textbf{0.385}& 18.35& 0.557& 0.357\\
        w/o $\mathcal{L}_\text{normal}$ & 15.41& \textbf{0.390}& 0.389& 17.86& 0.537& 0.375\\
        w/o $\mathcal{L}_{\text{depth}}, \mathcal{L}_{\text{normal}}$ & 15.21& 0.377& 0.397& 18.80& 0.568& 0.347\\
        
        \bottomrule
    \end{tabular}}
    \label{tab:ablation_loss}
    \vspace{-10pt}
    
\end{table}
